FibeR-CNN: Expanding Mask R-CNN to Improve Image-Based Fiber Analysis

Fiber-shaped materials (e.g. carbon nano tubes) are of great relevance, due to their unique properties but also the health risk they can impose. Unfortunately, image-based analysis of fibers still involves manual annotation, which is a time-consuming and costly process. We therefore propose the use of region-based convolutional neural networks (R-CNNs) to automate this task. Mask R-CNN, the most widely used R-CNN for semantic segmentation tasks, is prone to errors when it comes to the analysis of fiber-shaped objects. Hence, a new architecture - FibeR-CNN - is introduced and validated. FibeR-CNN combines two established R-CNN architectures (Mask and Keypoint R-CNN) and adds additional network heads for the prediction of fiber widths and lengths. As a result, FibeR-CNN is able to surpass the mean average precision of Mask R-CNN by 33 % (11 percentage points) on a novel test data set of fiber images.

==> tex/mainmatter/tab-dataset-comparison-aggregated.tex <==
% !TeX spellcheck = en_US

\begin{table*}
	\centering
	\caption{Data set properties, after aggregation (\identifierlegend/).}	
	\label{tab:DataSetComparisonAggregated}
	\begin{tabular}{ccccc|ccc|ccc}
		\toprule\toprule
		                                             \multicolumn{5}{c|}{}                                               &   \multicolumn{3}{c|}{\textbf{Number of Images}}   &  \multicolumn{3}{c}{\textbf{Number of Instances}}  \\
		\textbf{Loops} & \textbf{Clutter} & \textbf{Overlaps} & \textbf{Annotation} &        \textbf{Identifier}         & \textbf{Total} & \textbf{Training} & \textbf{Test} & \textbf{Total} & \textbf{Training} & \textbf{Test} \\
		      no       &        no        &        no         &       manual        &        \texttt{(-l|-c|-o)}         &   \num{236}    &     \num{200}     &   \num{36}    &   \num{250}    &     \num{211}     &   \num{39}    \\
		      no       &        no        &        yes        &       manual        &        \texttt{(-l|-c|+o)}         &   \num{107}    &     \num{90}      &   \num{17}    &   \num{227}    &     \num{192}     &   \num{35}    \\
		      no       &       yes        &        no         &       manual        &        \texttt{(-l|+c|-o)}         &   \num{351}    &     \num{298}     &   \num{53}    &   \num{444}    &     \num{379}     &   \num{65}    \\
		      no       &       yes        &        yes        &       manual        &        \texttt{(-l|+c|+o)}         &   \num{337}    &     \num{286}     &   \num{51}    &   \num{1014}   &     \num{855}     &   \num{159}   \\
		     yes       &      random      &      random       &       manual        &        \texttt{(+l|?c|?o)}         &    \num{44}    &     \num{35}      &    \num{9}    &    \num{75}    &     \num{59}      &   \num{16}    \\ \midrule
		    random     &      random      &      random       &      synthetic      & \texttt{(?l|?c|?o)}$_\text{synth}$ &   \num{500}    &     \num{425}     &   \num{75}    &   \num{760}    &     \num{645}     &   \num{115}   \\
		      no       &        no        &        no         &      semiautomatic      & \texttt{(-l|-c|-o)}$_\text{auto}$  &   \num{579}    &     \num{492}     &   \num{87}    &   \num{583}    &     \num{496}     &   \num{87}    \\ \bottomrule
	\end{tabular}
\end{table*}%

==> tex/mainmatter/tab-dataset-comparison.tex <==
% !TeX spellcheck = en_US

\begin{table*}
	\centering
	\caption{Data set properties (\identifierlegend/).}	
	\label{tab:DataSetComparison}
	\begin{tabular}{ccccc|ccc|ccc}
		\toprule\toprule
		                                             \multicolumn{5}{c|}{}                                               &   \multicolumn{3}{c|}{\textbf{Number of Images}}   &  \multicolumn{3}{c}{\textbf{Number of Instances}}  \\
		\textbf{Loops} & \textbf{Clutter} & \textbf{Overlaps} & \textbf{Annotation} &        \textbf{Identifier}         & \textbf{Total} & \textbf{Training} & \textbf{Test} & \textbf{Total} & \textbf{Training} & \textbf{Test} \\
		      no       &        no        &        no         &       manual        &        \texttt{(-l|-c|-o)}         &   \num{236}    &     \num{200}     &   \num{36}    &   \num{250}    &     \num{211}     &   \num{39}    \\
		      no       &        no        &        yes        &       manual        &        \texttt{(-l|-c|+o)}         &   \num{107}    &     \num{90}      &   \num{17}    &   \num{227}    &     \num{192}     &   \num{35}    \\
		      no       &       yes        &        no         &       manual        &        \texttt{(-l|+c|-o)}         &   \num{351}    &     \num{298}     &   \num{53}    &   \num{444}    &     \num{379}     &   \num{65}    \\
		      no       &       yes        &        yes        &       manual        &        \texttt{(-l|+c|+o)}         &   \num{337}    &     \num{286}     &   \num{51}    &   \num{1014}   &     \num{855}     &   \num{159}   \\
		     yes       &        no        &        no         &       manual        &        \texttt{(+l|-c|-o)}         &    \num{22}    &     \num{18}      &    \num{4}    &    \num{23}    &     \num{19}      &    \num{4}    \\
		     yes       &        no        &        yes        &       manual        &        \texttt{(+l|-c|+o)}         &    \num{2}     &      \num{1}      &    \num{1}    &    \num{5}     &      \num{3}      &    \num{2}    \\
		     yes       &       yes        &        no         &       manual        &        \texttt{(+l|+c|-o)}         &    \num{11}    &      \num{9}      &    \num{2}    &    \num{13}    &     \num{11}      &    \num{2}    \\
		     yes       &       yes        &        yes        &       manual        &        \texttt{(+l|+c|+o)}         &    \num{9}     &      \num{7}      &    \num{2}    &    \num{34}    &     \num{26}      &    \num{8}    \\ \midrule
		    random     &      random      &      random       &      synthetic      & \texttt{(?l|?c|?o)}$_\text{synth}$ &   \num{500}    &     \num{425}     &   \num{75}    &   \num{760}    &     \num{645}     &   \num{115}   \\
		      no       &        no        &        no         &      semiautomatic      & \texttt{(-l|-c|-o)}$_\text{auto}$  &   \num{579}    &     \num{492}     &   \num{87}    &   \num{583}    &     \num{496}     &   \num{87}    \\ \bottomrule
	\end{tabular}
\end{table*}%
